All-sky search for long-duration gravitational wave transients in the first Advanced LIGO observing run

We present the results of a search for long-duration gravitational wave transients in the data of the LIGO Hanford and LIGO Livingston second generation detectors between September 2015 and January 2016, with a total observational time of 49 days. The search targets gravitational wave transients of \unit[10 -- 500]{s} duration in a frequency band of \unit[24 -- 2048]{Hz}, with minimal assumptions about the signal waveform, polarization, source direction, or time of occurrence. No significant events were observed. %All candidate triggers were consistent with the expected background, As a result we set 90\% confidence upper limits on the rate of long-duration gravitational wave transients for different types of gravitational wave signals. We also show that the search is sensitive to sources in the Galaxy emitting at least $\sim$ \unit[$10^{-8}$]{$\mathrm{M_{\odot} c^2}$} in gravitational waves.

==> tabwvfs.tex <==
\begin{table}[!t]
\iffalse
\begin{tabular}{r|lllll|llll|ll|ll|ll|ll|ll|lll}
\hline
\hline
\multirow{2}{*}{Waveform} & \multicolumn{11}{c|}{Physical waveforms} & \multicolumn{11}{c|}{adhoc wavforms} \\
\cline{2-22}

 & ADI A & ADI B & ADI C & ADI D & ADI E & Magnetar D & Magnetar E & Magnetar F & Magnetar G & FA A & FA B & MONO A & MONO C & LINE A & LINE B & QUAD A & QUAD B & SG A & SG C & WNB A & WNB B & WNB C \\
\hline
Parameters & $M:5M_{\odot}$ & $M: 10M_{\odot}$ & $M: 10M_{\odot}$ & $M: 3M_{\odot}$ & $M: 8M_{\odot}$ & $\epsilon$: 0.005 & $\epsilon$: 0.01 & $\epsilon$: 0.5 & $\epsilon$: 0.08 & - & - & $f_{0}:$ 90 & $f_{0}:$ 405 & $f_{0}:$ 50 & $f_{0}:$ 900 & $f_{0}:$ 50 & $f_{0}:$ 405 & $f_{0}:$ 90 & $f_{0}:$ 405 & & \\

 & $a_{*}:0.30$ & $a_{*}:0.30$ & $a_{*}: 0.95$ & $a_{*}: 0.99$ & $f_{0}:$ 1598 & $f_{0}:$ 1171 & $f_{0}:$ 579 & $f_{0}:$ 405 & & & $\frac{|df}{dt}:$ 0.0 & $\frac{|df}{dt}:$ 0.0 & $\frac{|df}{dt}:$ 0.6 & $\frac{|df}{dt}:$ -2.0 & $\frac{|df}{dt}:$ 0.0 & $\frac{|df}{dt}:$ 0.0 & $\tau$ : 30 & $\tau$ : 50 & & \\

 & $\epsilon$:0.050 & $\epsilon$: 0.200 & $\epsilon$: 0.040 & $\epsilon$: 0.035 & $\epsilon$: 0.065 & & & & & & & $\frac{d^{2}f}{d^{2}t}:$ 0.00 & $\frac{d^{2}f}{d^{2}t}:$ 0.00 & $\frac{d^{2}f}{d^{2}t}:$ 0.00 & $\frac{d^{2}f}{d^{2}t}:$ 0.00 & $\frac{d^{2}f}{d^{2}t}:$ 0.33 $\frac{d^{2}f}{d^{2}t}:$ 0.04 & & & & & \\

Frequency band [Hz] &  135-166 & 110-209 & 130-251 & 119-173 & 111-234 & 1598-1900 & 1171-1900 & 579-950 & 400-490 & 1200-1500 & 800-1075 & 90 & 405 & 90-200 & 700-900 & 50-200 & 500-600 & 90 & 405 & 50-400 &  300-350 & 700-750 \\

Duration [s] & 39 & 9 & 236 & 142 & 76 & 400 & 400 & 400 & 400 & 25 & 197 & 150 & 250 & 250 & 100 & 30 & 70 & 150 & 250 & 20 & 60 & 100 \\

\hline
\hline
\end{tabular}
\fi

\begin{tabular}{|l|r|r|r||l|r|r|r|}
\hline
Name     & Param.           & Dur.     & Freq.      & Name      & Param.               & Dur.  & Freq \\
         &                  &      [s] &       [Hz] &           &                          &       [s] &       [Hz]\\
\hline
ADI A     & M=5\msun        &  39      &   135-166   & MONO     & $f_{0}$=90                & 150      & 90 \\
          & $a_{*}$=0.30     &          &             & A        & $\frac{df}{dt}$=0        &          &    \\              
          & $\epsilon$=0.05 &          &             &          & $\frac{d^{2}f}{d^{2}t}$=0  &          &    \\     
\hline
ADI B     & M=10\msun       &   9      &   110-209    & MONO    & $f_{0}$=405               & 250      & 405 \\
          & $a_{*}$=0.95     &          &              & C       & $\frac{df}{dt}$= 0       &          &     \\              
          & $\epsilon$=0.2  &          &              &         & $\frac{d^{2}f}{d^{2}t}$=0  &          &     \\     
\hline
ADI C     & M=10\msun       & 236     &   130-251     &  LINE A    & $f_{0}$=50                & 250 &   90-200  \\ 
          & $a_{*}$=0.95     &         &              &             & $\frac{df}{dt}$=0.6      &     &\\               
          & $\epsilon$=0.04 &         &               &            & $\frac{d^{2}f}{d^{2}t}$= 0 &  &\\      
\hline                                                        
ADI D     & M=\msun          & 142    &   119-173     &  LINE B     & $f_{0}$=900              & 100 & 700-900 \\ 
          & $a_{*}$=0.7       &        &              &              & $\frac{df}{dt}$= -2     &     &\\               
          & $\epsilon$=0.035 &        &               &             & $\frac{d^{2}f}{d^{2}t}$=0 &  &\\
\hline
ADI E     & M=8\msun         &  76    &   111-234     &  QUAD     & $f_{0}$=50                    &  30  & 50-200 \\  
          & $a_{*}$=0.99      &        &               &  A        & $\frac{df}{dt}$= 0          &      &\\                
          & $\epsilon$=0.065 &        &               &            & $\frac{d^{2}f}{d^{2}t}$= 0.33 & &\\       
\hline
magnetar& $\epsilon$= 0.005  & 400    & 1598-1900     &  QUAD     & $f_{0}$=500                  &  70  & 500-600 \\  
D          & $f_{0}$= 1598    &        &               &  B        & $\frac{df}{dt}$=0           &      &\\                 
magnetar& $\epsilon$= 0.01,  & 400    & 1171-1900     &            & $\frac{d^{2}f}{d^{2}t}$=0.04 & &\\       
\cline{5-8}
E          & $f_{0}$=1171     &        &               &  SG A      & $f_{0}$=90             & 150 & 90 \\
\cline{1-4}
magnetar& $\epsilon$=0.5     & 400    & 579-950       &            & $\tau$=30             &     &\\
\cline{5-8}
F          & $f_{0}$=579     &        &                &  SG C      & $f_{0}$=405            & 250 & 405 \\
\cline{1-4}
magnetar& $\epsilon$=0.08   & 400    & 400-490       &             & $\tau=$ 50           &     &\\
\cline{5-8}
G          & $f_{0}$=405     &        &               &  WNB A   & -                  &  20 &    50-400 \\
\hline                                            
FA A      & -                  &  25 & 1200-1500     &    WNB B     & -                  &  60 &   300-350 \\
\hline
FA B      & -                  & 197 &  800-1075     &    WNB C     & -                  & 100 &   700-750 \\
\hline









\hline














\hline
\end{tabular}

\caption{List of waveforms used to test the sensitivity of the search. For more details concerning the adhoc parameters see \cite{Abbott:2015vir}.}
\label{table:LT_wvf}
\end{table}


